Quantum-Classical Computing via Tensor Networks

Circuit knitting offers a promising path to the scalable execution of large quantum circuits by breaking them into smaller sub-circuits whose output is recombined through classical postprocessing. However, current techniques face excessive overhead due to a naive postprocessing method that neglects potential optimizations in the circuit structure. To overcome this, we introduce qTPU, a framework for scalable hybrid quantum-classical processing using tensor networks. By leveraging our hybrid quantum circuit contraction method, we represent circuit execution as the contraction of a hybrid tensor network (h-TN). The qTPU compiler automates efficient h-TN generation, optimizing the balance between estimated error and postprocessing overhead, while the qTPU runtime supports large-scale h-TN contraction using quantum and classical accelerators. Our evaluation shows orders-of-magnitude reductions in postprocessing overhead, a $10^4\times$ speedup in postprocessing, and a 20.7$\times$ reduction in overall runtime compared to the state-of-the-art Qiskit-Addon-Cutting (QAC).

==> Backup.tex <==
% \documentclass[10pt,conference]{IEEEtran}
% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage[hyphens]{url}
% \usepackage{fancyhdr}
% \usepackage{hyperref}


% % Ensure letter paper
% \pdfpagewidth=8.5in
% \pdfpageheight=11in

% \newcommand{\hpcayear}{2024}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%% -- UPDATE -- %%%%%%%%%%%%%%%
% \newcommand{\hpcasubmissionnumber}{NaN}
% \title{\projecttitle: A Quantum Tensor Processing Unit}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%% -- ONLY FOR CAMERA READY -- %%%%%%%%
% %\def\hpcacameraready{} % Uncomment to build camera-ready version
% \newcommand{\hpcapubid}{0000--0000/00\$00.00}
% \newcommand\hpcaauthors{First Author$\dagger$ and Second Author$\ddagger$}
% \newcommand\hpcaaffiliation{First Affiliation$\dagger$, Second Affiliation$\ddagger$}
% \newcommand\hpcaemail{Email(s)}

% %%%%% -- ARTEFACT EVALUATION RESULTS -- %%%%%%
% % Uncomment the following based on the badges that were awarded to this paper
% %\def\aeopen{}           % The artifact is publically available
% %\def\aereviewed{}     % The artefact has been reviewed
% %\def\aereproduced{} % The results have been reproduced
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % \input{space-tricks.tex}
% \input{mac.tex}


% \newcommand{\projecttitle}{\textsc{qTPU}}

% \usepackage{braket}
% \usepackage{tcolorbox}

% \usepackage{pifont}


% \newcommand{\cmark}{\ding{51}} % checkmark
% \newcommand{\xmark}{\ding{55}} % crossmark
% % \usepackage{listings}

% \usepackage{grumble}

% \input{hpca-template}



% \tcbset{
%     mybox/.style={
%         % colback=blue!5!white,   % Background color
%         % colframe=blue!75!black, % Frame color
%         fonttitle=\bfseries,    % Title font
%         title=Heading,          % Box title
%         width=\linewidth,       % Box width
%         % boxrule=0.5mm,          % Border thickness
%         % arc=4mm,                % Corner rounding
%         auto outer arc,         % Automatic outer arc
%         % boxsep=1mm,             % Separation between box and content
%     }
% }



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%% -- PAPER CONTENT STARTS -- %%%%%%%%%

% \begin{abstract}
% \input{sections/abstract}
% \end{abstract}

% \input{sections/introduction}
% \input{sections/background}
% \input{sections/overview}
% \input{sections/idea}
% \input{sections/compiler}
% \input{sections/knitter}
% % \input{sections/implementation}
% \input{sections/evaluation}
% \input{sections/related_work}
% \input{sections/conclusion}

% %%%%%%% -- PAPER CONTENT ENDS -- %%%%%%%%


% %%%%%%%%% -- BIB STYLE AND FILE -- %%%%%%%%
% \bibliographystyle{IEEEtranS}
% \bibliography{references}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \end{document}



==> ano_main.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Template for ASPLOS papers.
% %
% % History:
% % 
% % ASPLOS originally used jpaper.cls for submission but required acmart.cls for the
% % final camera-ready version. To avoid a change in format, starting ASPLOS 2024 Fall 
% % cycle, both the submission and the camera-ready versions started using acmart.cls.
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % use the base acmart.cls version 1.92
% % use the sigplan proceeding template with the default 10 pt fonts
% % nonacm option removes ACM related text in the submission. 
% \documentclass[nonacm,sigplan]{acmart}

% % enable page numbers
% \settopmatter{printfolios=true}

% % make references clickable 
% \usepackage[]{hyperref}


% \input{space-tricks.tex}
% \input{mac.tex}
% \newcommand{\projecttitle}{\textsf{qTPU}}

% \newcommand{\takeawaybox}[1]{%
%   \vspace{2pt}
%   \noindent
%   \framebox[1.0\columnwidth][l]{%
%     \parbox[b]{0.95\columnwidth}{%
%       #1  
%     }
%   }
%   \vspace{2pt}
% }


% \usepackage{listings}
% \usepackage{grumble}
% \usepackage{braket}



% \begin{document}
% % \title{qTPU: A Quantum Tensor Processor Unit}
% %\title{qTPU: Hybrid Quantum-Classical Co-Processing using Tensor Networks}
% % \title{qTPU: A Quantum Tensor Processing Architecture}
% % \title{qTPU: A Hybrid Quantum-Tensor Processing Unit}
% % \title{qTPU: Hybrid Quantum-Classical Processing\\ using Tensor Networks}
% % \title{Quantum-Classical Processing using Tensor Networks}
% \title{Quantum-Classical Computing via Tensor Networks}
% %\title{Quantum-Classical Computing\\ via Tensor Networks}
% % \title{qTPU: Scalable Quantum }
% % \title{Scalable Quantum-Classical Processing with Tensor Networks}

% % \author{Paper \#96}

% \begin{abstract}
%   \input{sections/abstract}
% \end{abstract}

% \maketitle % should come after the abstract
% \pagestyle{plain} % should come right after \maketitle


% \input{sections/introduction}
% \input{sections/background}
% \input{sections/overview}
% \input{sections/idea}
% \input{sections/compiler}
% \input{sections/knitter}
% % \input{sections/implementation}
% \input{sections/evaluation}
% \input{sections/related_work}
% \input{sections/conclusion}

% \bibliographystyle{unsrt}
% \bibliography{references}

% \end{document}



==> hpca-template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% -- DO NOT MODIFY -- %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\author{
  \ifdefined\hpcacameraready
    \IEEEauthorblockN{\hpcaauthors{}}
      \IEEEauthorblockA{
        \hpcaaffiliation{} \\
        \hpcaemail{}
      }
  \else
    \IEEEauthorblockN{\normalsize{HPCA \hpcayear{} Submission
      \textbf{\#\hpcasubmissionnumber{}}} \\
      \IEEEauthorblockA{
        Confidential Draft \\
        Do NOT Distribute!!
      }
    }
  \fi 
}

% Heading and footer for title page
\fancypagestyle{camerareadyfirstpage}{%
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[C]{
    \ifdefined\aeopen
    \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}    
    \else
      \ifdefined\aereviewed
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \ifdefined\aereproduced
      \parbox[][12mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
      \else
      \parbox[][0mm][t]{13.5cm}{\hpcayear{} IEEE International Symposium on High-Performance Computer Architecture (HPCA)}
    \fi 
    \fi 
    \fi 
    \ifdefined\aeopen 
      \includegraphics[width=12mm,height=12mm]{ae-badges/open-research-objects.pdf}
    \fi 
    \ifdefined\aereviewed
      \includegraphics[width=12mm,height=12mm]{ae-badges/research-objects-reviewed.pdf}
    \fi 
    \ifdefined\aereproduced
      \includegraphics[width=12mm,height=12mm]{ae-badges/results-reproduced.pdf}
    \fi
  }
  %\fancyfoot[L]{\hpcapubid{} \copyright \hpcayear{} IEEE}
  \fancyfoot[C]{}
}
% Heading and footer for remaining pages
\fancyhead{}
\renewcommand{\headrulewidth}{0pt}
%\fancyhead[C]{\hpcayear{} IEEE International Symposium on
% High-Performance Computer Architecture (HPCA)}



\begin{document}
\maketitle

%Enables the camera ready header and footer
\ifdefined\hpcacameraready 
  \thispagestyle{camerareadyfirstpage}
  \pagestyle{empty}
\else
  \thispagestyle{plain}
  \pagestyle{plain}
\fi

\newcommand{\hpcaheight}{0mm}
\ifdefined\eaopen
\renewcommand{\hpcaheight}{12mm}
\fi
  


==> sections/runtime.tex <==
\section{Runtime}

\subsection{Workflow}

\begin{enumerate}
    \item Instantiate all the fragments, only the needed instantiations
    \item Sample the fragments on a set of quantum devices
    \item Build a tensor network of the results
    \item Run a tensor network contraction of the results
\end{enumerate}

2 modes: Full prob distr reconstruction and construction of observables

Since expectation values are scalars, we can use GPUs to accelerate the tensor network.

\subsection{Tensor Network Creation}

\subsubsection*{Result Nodes}
Executing a circuit fragment yields $\prod_{j=0}^{n-1} |C_k|$ results with $n$ virtual gates in the respective fragment. To create the tensor node of each fragment, we build a tensor of $n$ dimensions, where the $j$-th dimension has the cardinality of $|C_j|$. Therefore, the result at index $(x, y, z)$ is the result where the fragment was in the $x$-th instantiation of the first virtual gate, ....

\subsubsection*{Coefficient Nodes}

\subsection{Optimal Tensor Network Contraction}



% \begin{table}[t]
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Framework} & \textbf{Knitting} & \textbf{WC/QPD} & \textbf{Hyper-Opt.} \\
% \hline
% CutQC \cite{tang2021cutqc} & $4^N$ & \cmark \xmark & \xmark  \\
% \hline
% CKT \cite{circuit-knitting-toolbox} & $\mathcal{O}(6^N)$ & \cmark  \cmark & \xmark  \\
% \hline
% ScaleQC \cite{tang2022scaleqc} & $4^{cc}$ & \cmark  \xmark & \xmark  \\
% \hline
% PLN \cite{lowe2023fast} & $4^{cc}$ & \cmark  \xmark & \xmark \\
% \hline
% \textbf{\projecttitle{}} & $\mathcal{O}(5^{cc})$ & \cmark  \cmark & \cmark \\
% \hline
% \end{tabular}
% \vspace{2pt}
% \label{table:comparison}
% \caption{Comparison to Circuit Knitting Baselines}
% \end{table}
